Real-time visualization of metastable charge regulation pathways in molecularly confined slit geometries

Transport of ions in molecular-scale confined spaces is central to all aspects of life and technology: into a crack, it may break steel within days; through a membrane separator, it determines the efficiency of electrochemical energy conversion devices; or through lipid membranes, it steers neural communication. Yet, the direct observation of ion mobility and structuring in sub-nanometer confinement is experimentally challenging and, so far, solely accessible to molecular simulations. Here, we show quantitative, 3D molecularly-resolved ion transportation of aqueous ionic liquid and s-block metal ion solutions, confined to electrochemically-modulated, molecular-sized slits. Our analysis of atomically resolved solid/liquid interface unveils generic rules of how enthalpic ion-ion and ion-surface interactions and entropic confinement effects determine the charge regulation mechanism. Altering our general understanding, the confined charge regulation may proceed via fast, kinetically favoured, metastable pathways, followed by slow diffusive thermodynamic ion reorganization, which has important implications for all charge-regulated systems.

==> MS114 - MSW 02 - IL gap upload arxiv 210402/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
